Relative dendroidal Rezk nerve and applications

We extend the dendroidal Rezk nerve to the setting of relative $\infty$-operads. Our main theorem relates it to localization of $\infty$-operads, generalizing a theorem of Mazel-Gee. By exploiting the relation, we obtain a surprisingly effective tool to prove localization results in operadic contexts. As applications, we obtain a number of new results on operadic localizations, including a generalization of Willwacher's recent result on cyclic operads and operadic modules, and a description of locally constant factorization algebras on spheres in terms of discrete geometry.

==> preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage{amsmath,amsthm,amssymb}
\usepackage[unicode=true,pdfusetitle,
 bookmarks=true,bookmarksnumbered=false,bookmarksopen=false,
 breaklinks=false,pdfborder={0 0 0},pdfborderstyle={},backref=false,colorlinks=false]
 {hyperref}
\usepackage{mathtools}
\usepackage{adjustbox}
\usepackage{enumitem}
\usepackage{xcolor}
\usepackage{eucal}
\usepackage{tikz}
\usetikzlibrary{arrows.meta, positioning, shapes, fit, shapes.geometric}
\usetikzlibrary{shapes.geometric, arrows}
\tikzstyle{sec} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]
\usepackage{mathrsfs}
\usepackage{stackrel}
\usepackage{mleftright}
\mleftright
\usepackage{upgreek}
\usepackage{wasysym} 


\usepackage{scalerel,stackengine}


\usepackage{mathalpha}

\RequirePackage{tikz-cd}
\tikzcdset{scale cd/.style={every label/.append style={scale=#1},
    cells={nodes={scale=#1}}}}
% `amssymb` is necessary for `\lrcorner` and `\ulcorner`.
\RequirePackage{amssymb}
% `calc` is necessary to draw curved arrows.
\usetikzlibrary{calc}
% `pathmorphing` is necessary to draw squiggly arrows.
\usetikzlibrary{decorations.pathmorphing}
% `spath3` is necessary to draw shortened edges.
\usetikzlibrary{spath3}

% A TikZ style for curved arrows of a fixed height, due to AndréC.
\tikzset{curve/.style={settings={#1},to path={(\tikztostart)
    .. controls ($(\tikztostart)!\pv{pos}!(\tikztotarget)!\pv{height}!270:(\tikztotarget)$)
    and ($(\tikztostart)!1-\pv{pos}!(\tikztotarget)!\pv{height}!270:(\tikztotarget)$)
    .. (\tikztotarget)\tikztonodes}},
    settings/.code={\tikzset{quiver/.cd,#1}
        \def\pv##1{\pgfkeysvalueof{/tikz/quiver/##1}}},
    quiver/.cd,pos/.initial=0.35,height/.initial=0}

% A TikZ style for shortening paths without the poor behaviour of `shorten <' and `shorten >'.
\tikzset{between/.style n args={2}{/tikz/execute at end to={
    \tikzset{spath/split at keep middle={current}{#1}{#2}}
}}}

% TikZ arrowhead/tail styles.
\tikzset{tail reversed/.code={\pgfsetarrowsstart{tikzcd to}}}
\tikzset{2tail/.code={\pgfsetarrowsstart{Implies[reversed]}}}
\tikzset{2tail reversed/.code={\pgfsetarrowsstart{Implies}}}
% TikZ arrow styles.
\tikzset{no body/.style={/tikz/dash pattern=on 0 off 1mm}}

%%%%%%%%%%%%%%%%%%%% NEW MATHCAL \mathcalpxtx
%\DeclareMathAlphabet{\mathdutchcal}{U}{dutchcal}{m}{n}

%%%%%%%%%%%%%%%%%% NEW MATHBB
\DeclareFontFamily{U}{stixtwobb}{\skewchar\font=45}%
\DeclareFontShape{U}{stixtwobb}{m}{n}{<->\mathalfa@bbscaled stix2-mathbb}{}
\DeclareMathAlphabet{\mathbbst}{U}{stixtwobb}{m}{n}

%theorems
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\theoremstyle{plain}
\newtheorem{thm}[equation]{Theorem}
\theoremstyle{definition}
\newtheorem{convention}[equation]{Convention}
\theoremstyle{definition}
\newtheorem{defn}[equation]{Definition}
\theoremstyle{definition}
\newtheorem{notation}[equation]{Notation}
\theoremstyle{remark}
\newtheorem{rem}[equation]{Remark}
\theoremstyle{plain}
\newtheorem{prop}[equation]{Proposition}
\theoremstyle{plain}
\newtheorem{cor}[equation]{Corollary}
\theoremstyle{plain}
\newtheorem*{conj}{Conjecture}
\newtheorem*{prop*}{Proposition}

\newtheorem{lem}[equation]{Lemma}
\theoremstyle{definition}
\newtheorem{example}[equation]{Example}
%for comments
\newcommand{\notehelper}[3]{\textcolor{#3}{$\blacksquare$}\marginpar{\ifodd\thepage\raggedright\else\raggedleft\fi\color{#3}\tiny \textbf{#2:} #1}}
\newcommand\francesca [1]{\notehelper{#1}{Francesca}{orange}}
\newcommand\victor [1]{\notehelper{#1}{Victor}{blue}}
\newcommand\ken[1]{\notehelper{#1}{Ken}{magenta}}

\usepackage{cancel}
\newcommand{\fnew}[1]{{\color{orange}{#1}}}
\newcommand{\vnew}[1]{{\color{blue}{#1}}}
\newcommand{\knew}[1]{{\color{magenta}{#1}}}


%\newcommand{\fremove}[1]{\ifmmode{\fnew{\underline{$#1$}}}\else\fnew{\underline{#1}}\fi}
%\newcommand{\fremove}[1]{\fnew{\underline{#1}}}

\usepackage[normalem]{ulem}
\newcommand{\fremove}[1]{\fnew{\uline{#1}}}
\newcommand{\kremove}[1]{\knew{\uline{#1}}}
\newcommand{\vremove}[1]{\vnew{\uline{#1}}}


\newcommand{\brbinom}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}


 % customTheorem for the intro
\theoremstyle{plain}
\newtheorem{customthm}{Theorem}
\renewcommand{\thecustomthm}{\Alph{customthm}} 

% customCor for the intro
\newtheorem{customcor}[customthm]{Corollary}


% customConvention for the intro
\theoremstyle{plain}
\newtheorem{customcon}{Convention}
\renewcommand{\thecustomcon}{\Alph{customcon}} 


%macros
\newcommand{\pr}[1]{\left(#1\right)}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\ps}[3]{%
  {\vphantom{}{}_{#2}}{#1}{_{#3}}%
}
\newcommand{\cat}[1]{\mathcal{#1}}
\newcommand{\inp}[1]{\langle #1 \rangle}

\newcommand{\curlyCatinfty}{\mathcal{C}\mathrm{at}_{\infty}}
% \newcommand{\curlyGpdinfty}{\mathrm{Gpd}_{\infty}}
\newcommand{\curlyOpinfty}{\mathcal{O}\mathrm{p}_{\infty}}
\newcommand{\curlyRelCatinfty}{\mathcal{R}\mathrm{el}\mathcal{C}\mathrm{at}_{\infty}}
\newcommand{\curlyRelOpinfty}{\mathcal{R}\mathrm{el}\mathcal{C}\mathrm{at}_{\infty}}
\newcommand{\Cart}{\mathcal{C}\mathrm{art}}

\newcommand{\RelCatinfty}{\mathcal{R}\mathrm{el}\mathcal{C}\mathrm{at}_{\infty}}
\newcommand{\RelOpinfty}{\mathcal{R}\mathrm{el}\mathcal{O}\mathrm{p}_{\infty}}
\newcommand{\Catinfty}{\mathcal{C}\mathrm{at}_{\infty}}
\newcommand{\Opinfty}{\mathcal{O}\mathrm{p}_{\infty}}

\newcommand{\QCat}{\mathrm{QCat}}
\newcommand{\Set}{\mathrm{Set}}
\newcommand{\sSet}{\mathrm{sSet}}
\newcommand{\dSet}{\mathrm{dSet}}
\newcommand{\sfCSS}{\mathrm{CSS}}


%\newcommand{\Cat}{\mathrm{Cat}}
%%relative version
\newcommand{\Cat}{\mathcal{C}\mathrm{at}}


\newcommand{\DQOp}{\mathrm{DQOp}}
\newcommand{\LQOp}{\mathrm{LQOp}}
\newcommand{\CDSS}{\mathrm{CDSS}}
\newcommand{\Rel}{\mathcal{R}\mathrm{el}}
\newcommand{\Op}{\mathcal{O}\mathrm{p}}
%%relative version
%\newcommand{\Op}{\mathcal{O}\mathrm{p}}


\newcommand{\RelOp}{\mathcal{R}\mathrm{el}\mathcal{O}\mathrm{p}}
\newcommand{\OpdMod}{\mathrm{OpdMod}}
\newcommand{\Cyc}{\mathrm{Cyc}}
\newcommand{\FB}{\mathrm{FB}}
\newcommand{\Fin}{\mathrm{Fin}}

\newcommand{\Lurie}{\mathrm{Lurie}}
\newcommand{\Rezk}{\mathrm{Rezk}}
\newcommand{\hc}{\mathrm{hc}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\dend}{\mathrm{dend}}
\newcommand{\Kan}{\mathrm{Kan}}
\newcommand{\pt}{\mathrm{pt}}
\newcommand{\opd}{\mathrm{opd}}
\global\long\def\mod{\mathrm{mod}}%

\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\Map}{\operatorname{Map}}
\newcommand{\qAlg}{\operatorname{Alg}}
\newcommand{\Leaf}{\operatorname{Leaf}}
\global\long\def\Vert{\operatorname{Vert}}%
\newcommand{\In}{\operatorname{In}}
\newcommand{\Adj}{\operatorname{Adj}}
\newcommand{\Edge}{\operatorname{Edge}}
\newcommand{\Alg}{\operatorname{Alg}}
\newcommand{\colim}{\operatorname{colim}}

\newcommand{\Del}{\Delta}
\newcommand{\Den}{\Omega}

\newcommand{\op}{\mathrm{op}}
\newcommand{\from}{\colon}
\newcommand{\N}{\mathrm{N}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\ev}{\mathrm{ev}}
\newcommand{\act}{\mathrm{act}}
\newcommand{\hoeq}{\mathrm{hoeq}}
\newcommand{\weq}{\mathrm{weq}}

\global\long\def\t{\otimes}%

%  kalligraphische Buchstaben
\newcommand{\dN}{\mathrm{N}_\mathrm{d}}
\newcommand{\dNR}{\mathrm{N}^_\mathrm{d}}
\setcounter{tocdepth}{1}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}

%complete Segal space localization functor
\newcommand{\OO}{\mathbb{O}}
% \newcommand{\CS}{{\cC\cS}}


%%Start adjunction

\usepackage{pict2e} 
\makeatletter
\newcommand{\adjunction}[4]{%
	% #1 : #2 <arrows> #3 : #4
	#1\colon #2%
	\mathrel{\vcenter{%
			\offinterlineskip\m@th
			\ialign{%
				\hfil$##$\hfil\cr
				\longrightharpoonup\cr
				\noalign{\kern-.3ex}
				\smallbot\cr
				\longleftharpoondown\cr
			}%
	}}%
	#3 \noloc #4%
}
\newcommand{\longrightharpoonup}{\relbar\joinrel\rightharpoonup}
\newcommand{\longleftharpoondown}{\leftharpoondown\joinrel\relbar}
\newcommand\noloc{%
	\nobreak
	\mspace{6mu plus 1mu}
	{:}
	\nonscript\mkern-\thinmuskip
	\mathpunct{}
	\mspace{2mu}
}
\newcommand{\smallbot}{%
	\begingroup\setlength\unitlength{.15em}%
	\begin{picture}(1,1)
		\roundcap
		\polyline(0,0)(1,0)
		\polyline(0.5,0)(0.5,1)
	\end{picture}%
	\endgroup
}
\makeatother
%%End adjunction


\usepackage{contour}
\usepackage{ulem}

\renewcommand{\ULdepth}{1.8pt}
\contourlength{1.3pt}

\newcommand{\myuline}[1]{%
	\uline{\phantom{#1}}%
	\llap{\contour{white}{#1}}%
}

\newcommand{\uALG}{\mbox{\myuline{$\Alg$}}}


%\definecolor{darkred}{rgb}{0.8,0.1,0.1}

%\hypersetup{
%	colorlinks=true,         % false: boxed links; true: colored links,false is default
%	urlcolor=darkred, %blue??
%	linkcolor=darkred,
%	citecolor=darkred,
%}

\bibliographystyle{plainurl}



